Physics at a 100 TeV pp collider: beyond the Standard Model phenomena

This report summarises the physics opportunities in the search and study of physics beyond the Standard Model at a 100 TeV pp collider.

==> 01-SUSY/secminisplit.tex <==

  
  \subsection{Mini-Split SUSY}
It may be that some of the SUSY partners are heavy and lie beyond the kinematic reach of the FCC-hh, while others may be light enough to be observed.  In fact, one scenario, known as ``Split Supersymmetry'' has been considered for some time \cite{}.  In this scenario some of the attractive features of SUSY are retained, including as gauge coupling unification and the realisation of a viable dark matter candidate, by keeping the gauginos and the Higgsinos near the weak scale while raising the scalar superpartner masses well above this scale.  This spectrum can be motivated by specific SUSY breaking scenarios, such as anomaly mediation, or by imposing an R-symmetry on the theory which is only broken at the weak scale, justifying the hierarchy between the SUSY breaking scalar masses and the SUSY breaking gaugino masses.  This picture necessarily invokes fine-tuning to retain one light scalar (the Higgs) however there are arguments as to why such fine tuning may arise in nature \cite{}.

The discovery of the Higgs boson and the precise measurement of the Higgs boson mass has increased the attraction of the Split SUSY scenario. In the MSSM it is not possible to raise the Higgs mass to $m_h \sim 125$ GeV without requiring significant fine tuning and at least one heavy stop squark.  Embracing this tuning the compelling picture of the ``Mini-Split'' scenario \cite{} is raised, where the other scalars, including the stop squarks, may have mass in the range $\mathcal{O}(\text{few}) \lesssim m_{\tilde{t}} \lesssim 10^{5}$ TeV while the gauginos and Higgsinos may lie within reach of the FCC-hh.  This possibility is...

\subsubsection{Jung, Wells: Mini-Split Gauginos}
The spectrum of split supersymmetry (SUSY) contains lighter gauginos (bino, winos, gluinos) and heavier scalars (sfermions and Higgs bosons)~\cite{Wells:2003tf,ArkaniHamed:2004fb,Giudice:2004tc,Wells:2004di}. Among the gauginos, gluino production can be a useful way to search for split SUSY  at hadron colliders. Pure wino production is smaller by electroweak couplings. Pure bino production is very small since it has no direct couplings to gauge bosons. Unless gluinos are much heavier than other gauginos, gluino production can be the dominant production mode of split SUSY particles. In this section, we sutdy gluino search propects at a 100 TeV $pp$ collider in split SUSY models~\cite{Jung:2013zya,Cohen:2013xda}.

Gluinos are pair produced at $pp$ colliders. Once produced, each gluino subsequently decays to the lightest gauginos (LSP) -- winos or binos -- via off-shell squarks as
\begin{equation}
\widetilde{g} \to \chi_1^0 j j.
\label{eq:decmode} \end{equation}
Pair production of gluinos then yields $\widetilde{g} \widetilde{g} \to \chi_1^0 \chi_1^0 jjjj$. This channel can be searched using an effective mass variable, $M_{\rm eff}$. The effective mass is defined as a scalar sum
\begin{equation}
M_{\rm eff} =  \sum_i p_T(i) + E_T^{\rm miss},
\end{equation}
where the sum runs over all jets with $p_T>50$ GeV and $\eta <5.0$. Cuts on the data that aid selecting signal over background include (see also~\cite{Hinchliffe:2001bz}):
\begin{itemize}
\item At least two jets with $p_T > 0.1\, M_{\rm eff}$.
\item Lepton veto.
\item $E_T^{\textrm{miss}} > 0.2 M_{\rm eff}$ and $p_T(j_1) < 0.35\, M_{\rm eff}$.
\item $\Delta \phi(j_1,E_T^{\textrm{miss}}) < \pi -0.2$ and $\Delta \phi(j_1,j_2)<2\pi/3$
\item $M_{\rm eff}> 1.5 M_{\widetilde{g}}$.
\end{itemize}
The $M_{\rm eff}$ spectrum depends only on the gluino mass and not on the LSP mass, as long as the gluino is more than 3 times heavier than the LSP~\cite{Jung:2013zya}. The discovery prospect in terms of the gluino mass is shown in Fig.\ref{fig:reach-glupair}; the integrated luminosity needed for $5\sigma$ statistical significance is shown. 

%
\begin{figure}
\centerline{
\includegraphics[width=0.49\columnwidth]{BSM_SUSY_figures/reach-glupair.pdf} 
\includegraphics[width=0.49\columnwidth]{BSM_SUSY_figures/mratio-reach.pdf} 
}
\caption{{\bf (Left):} The integrated luminosity (fb$^{-1}$) needed to discover gluino pairs in split SUSY models with $5\sigma$ statistical significance is contour plotted~\cite{Jung:2013zya}. It is assumed that the gluino is more than 3 times heavier than the LSP so that the $M_{\rm eff}$ analysis is valid. In the upper horizontal axis, the wino mass with the minimal AMSB relation is also shown. {\bf (Right):} The result at a 100 TeV $pp$ collider is shown in terms of the gluino-to-LSP mass ratio in split SUSY~\cite{Jung:2013zya}. Blue and red regions are predictions of AMSB models with squark masses and $\tan \beta$ varied. See text and Ref.~\cite{Jung:2013zya} for more details.}
\label{fig:reach-glupair}
\end{figure}
%

The results can be interpreted in three ways. First, at a 100 TeV $pp$ collider, up to about 7 (13) TeV gluinos can be discovered with 10 (1000) fb$^{-1}$ of data. This result applies to any split SUSY models as long as the gluino is 3 times heavier than the LSP and the decay mode in eq.(\ref{eq:decmode}) is dominant; for a smaller mass difference between the gluino and the LSP, the $M_{\rm eff}$ becomes a less useful observable for discovery and other strategies may be needed.

Secondly, if the minimal anomaly-mediated SUSY breaking (AMSB) model~\cite{Randall:1998uk,Giudice:1998xp} is considered as a particular example of split SUSY models, the reach on the gluino mass can be interpreted simultaneously as a reach on the mass of the wino dark matter candidate. In the minimal AMSB model, the wino is the LSP; squarks are one-loop factor heavier than the gluino and out of reach for the collider. The gluino-to-wino mass ratio, which is key to this interpretation of an indirect wino bound, is almost fixed, but varies from 8 to 9.5 for the wino mass between 3 TeV and 200 GeV, respectively~\cite{Jung:2013zya}. The variation is almost entirely due to the running of gauge couplings, and the Higgsino contribution to the quantum correction can be ignored. The wino mass corresponding to the gluino mass in this model is also shown in the upper horizontal axis in left panel of Fig.\ref{fig:reach-glupair}. A 100 TeV $pp$ collider can probe wino mass up to 900 GeV (1.4 TeV)  with 10 (1000) fb$^{-1}$ of integrated luminosity. It is known that the $\sim 3$ TeV pure wino can be a thermal dark matter contributing to full dark matter density~\cite{Hisano:2006nn}, but astrophysical constraints may rule out this possibility~\cite{Cohen:2013ama,Fan:2013faa}. In any event, this very large wino mass is too heavy to be probed at a 100 TeV collider, yet a smaller wino mass, perhaps as a non-thermal dark matter source, can be indirectly probed to mass scales above a TeV as seen by this analysis.


Finally, the result can be interpreted more generally in terms of the reach on the gluino-to-LSP mass ratio. This is done in the right panel of Fig.\ref{fig:reach-glupair}. The aforementioned minimal AMSB relation of the gluino and wino masses can be modified in general split SUSY models. The variations of sfermion masses between $1 \leq m_{\widetilde{f}} / m_{\widetilde{g}} \leq 4\pi \alpha_S$ and $3 \leq \tan \beta \leq 50$ with $|\mu|=4$ TeV lead to the blue and red regions; heavy squarks and Higgsinos modify the gluino mass and the wino mass at one-loop order, respectively. The dependence on the renormalization scale is much smaller. The region of $M_{\rm LSP}$ and $M_{\tilde g}/M_{\rm LSP}$ probed is under the integrated lumonsity contours in the figure. For more details of each curve, we refer to Ref.~\cite{Jung:2013zya}. This interpretation is most useful when a certain split SUSY model predicts a certain gaugino mass ratio.



==> 02-DM/DM_BSM_portal_1/HKSW_bib.tex <==
\bibliography{ref}
\bibliographystyle{ArXiv}
\begin{thebibliography}{99}

%\cite{Planck:2015xua}
\bibitem{Planck:2015xua}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2015 results. XIII. Cosmological parameters,''
  arXiv:1502.01589 [astro-ph.CO].
  %%CITATION = ARXIV:1502.01589;%%
  
%\cite{Bertone:2004pz}
\bibitem{Bertone:2004pz}
  G.~Bertone, D.~Hooper and J.~Silk,
  %``Particle DM: Evidence, candidates and constraints,''
  Phys.\ Rept.\  {\bf 405} (2005) 279
  [hep-ph/0404175].
  %%CITATION = HEP-PH/0404175;%%
  
\bibitem{FCC}
M. Benedikt, ``FCC study overview and status'', talk at the FCC week
2015, Washington D.C., 23-29 March 2015, \hfill \\
{ \tt http://indico.cern.ch/event/340703/session/108/contribution/186}
\\
D. Schulte, ``FCC-hh machine overview'' , {\it ibidem}, \hfill \\
{\tt http://indico.cern.ch/event/340703/session/109/contribution/189}
\\
CEPC/SppC preliminary conceptual design report,
{\tt http://cepc.ihep.ac.cn/preCDR/volume.html}
  
  
%\cite{Harris:2014hga}
\bibitem{Harris:2014hga}
  P.~Harris, V.~V.~Khoze, M.~Spannowsky and C.~Williams,
  %``Constraining Dark Sectors at Colliders: Beyond the Effective Theory Approach,''
  Phys.\ Rev.\ D {\bf 91} (2015) 5,  055009
  [arXiv:1411.0535 [hep-ph]].
  %%CITATION = ARXIV:1411.0535;%%
  
   %\cite{Low:2014cba}
\bibitem{Low:2014cba}
  M.~Low and L.~T.~Wang,
  %``Neutralino DM at 14 TeV and 100 TeV,''
  JHEP {\bf 1408} (2014) 161
  [arXiv:1404.0682 [hep-ph]].
  %%CITATION = ARXIV:1404.0682;%%
  
  %\cite{Bramante:2014tba}
\bibitem{Bramante:2014tba}
  J.~Bramante, P.~J.~Fox, A.~Martin, B.~Ostdiek, T.~Plehn, T.~Schell and M.~Takeuchi,
  %``Relic neutralino surface at a 100 TeV collider,''
  Phys.\ Rev.\ D {\bf 91} (2015) 5,  054015
  [arXiv:1412.4789 [hep-ph]].
  %%CITATION = ARXIV:1412.4789;%%
 
%\cite{Xiang:2015lfa}
\bibitem{Xiang:2015lfa} 
  Q.~F.~Xiang, X.~J.~Bi, P.~F.~Yin and Z.~H.~Yu,
  %``Searches for DM signals in simplified models at future hadron colliders,''
  Phys.\ Rev.\ D {\bf 91}, 095020 (2015)
  [arXiv:1503.02931 [hep-ph]].
  %%CITATION = ARXIV:1503.02931;%%
  %2 citations counted in INSPIRE as of 31 Aug 2015
  
  %\cite{Freitas:2015hsa}
\bibitem{Freitas:2015hsa} 
  A.~Freitas, S.~Westhoff and J.~Zupan,
  %``Integrating in the Higgs Portal to Fermion DM,''
  JHEP {\bf 1509}, 015 (2015)
  [arXiv:1506.04149 [hep-ph]].
  %%CITATION = ARXIV:1506.04149;%%
  %4 citations counted in INSPIRE as of 23 Oct 2015
  
  %\cite{Cirelli:2014dsa}
\bibitem{Cirelli:2014dsa} 
  M.~Cirelli, F.~Sala and M.~Taoso,
  %``Wino-like Minimal DM and future colliders,''
  JHEP {\bf 1410}, 033 (2014)
  [JHEP {\bf 1501}, 041 (2015)]
  [arXiv:1407.7058 [hep-ph]].
  %%CITATION = ARXIV:1407.7058;%%
  %38 citations counted in INSPIRE as of 23 Oct 2015
  
  %\cite{Abdallah:2014hon}
\bibitem{Abdallah:2014hon}
  J.~Abdallah {\it et al.},
 % ``Simplified Models for DM and Missing Energy Searches at the LHC,''
  arXiv:1409.2893 [hep-ph].
  %%CITATION = ARXIV:1409.2893;%%

%\cite{Malik:2014ggr}
\bibitem{Malik:2014ggr}
  S.~Malik {\it et al.},
%  ``Interplay and Characterization of DM Searches at Colliders and in Direct Detection Experiments,''
  arXiv:1409.4075 [hep-ex].
  %%CITATION = ARXIV:1409.4075;%%
  
%\cite{Buchmueller:2014yoa}
\bibitem{Buchmueller:2014yoa} 
  O.~Buchmueller, M.~J.~Dolan, S.~A.~Malik and C.~McCabe,
  %``Characterising DM searches at colliders and direct detection experiments: Vector mediators,''
  JHEP {\bf 1501}, 037 (2015)
  [arXiv:1407.8257 [hep-ph]].
  %%CITATION = ARXIV:1407.8257;%%
  %39 citations counted in INSPIRE as of 31 Aug 2015

%\cite{Buckley:2014fba}
\bibitem{Buckley:2014fba} 
  M.~R.~Buckley, D.~Feld and D.~Goncalves,
  %``Scalar Simplified Models for DM,''
  arXiv:1410.6497 [hep-ph].
  %%CITATION = ARXIV:1410.6497;%%
  
 %\cite{Haisch:2015ioa}
\bibitem{Haisch:2015ioa}
  U.~Haisch and E.~Re,
  %``Simplified DM top-quark interactions at the LHC,''
  arXiv:1503.00691 [hep-ph].
  %%CITATION = ARXIV:1503.00691;%% 
  
 %\cite{Chala:2015ama}
\bibitem{Chala:2015ama}
  M.~Chala, F.~Kahlhoefer, M.~McCullough, G.~Nardini and K.~Schmidt-Hoberg,
  %``Constraining Dark Sectors with Monojets and Dijets,''
  arXiv:1503.05916 [hep-ph].
  %%CITATION = ARXIV:1503.05916;%% 
  
 %\cite{Khoze:2015sra}
\bibitem{Khoze:2015sra}
  V.~V.~Khoze, G.~Ro and M.~Spannowsky,
  %``Spectroscopy of Scalar Mediators to DM at the LHC and at 100 TeV,''
  arXiv:1505.03019 [hep-ph].
  %%CITATION = ARXIV:1505.03019;%%
  
  %\cite{Buchmueller:2015eea}
\bibitem{Buchmueller:2015eea}
  O.~Buchmueller, S.~A.~Malik, C.~McCabe and B.~Penning,
  %``Constraining the Fermi-LAT excess with multi-jet plus MET collider searches,''
  arXiv:1505.07826 [hep-ph].
  %%CITATION = ARXIV:1505.07826;%%
  %1 citations counted in INSPIRE as of 11 Aug 2015
  
  %\cite{Fan:2015sza}
\bibitem{Fan:2015sza}
  J.~Fan, S.~M.~Koushiappas and G.~Landsberg,
  %``Pseudoscalar Portal DM and New Signatures of Vector-like Fermions,''
  arXiv:1507.06993 [hep-ph].
  %%CITATION = ARXIV:1507.06993;%%
  
  %\cite{Lebedev:2014bba}
\bibitem{Lebedev:2014bba} 
  O.~Lebedev and Y.~Mambrini,
  %``Axial DM: The case for an invisible $Z?$,''
  Phys.\ Lett.\ B {\bf 734}, 350 (2014)
  [arXiv:1403.4837 [hep-ph]].
  %%CITATION = ARXIV:1403.4837;%%
  %25 citations counted in INSPIRE as of 23 Oct 2015
  
  %\cite{Abdallah:2015ter}
\bibitem{Abdallah:2015ter}
  J.~Abdallah {\it et al.} [DM@LHC],
  %``Simplified Models for DM Searches at the LHC,''
  arXiv:1506.03116 [hep-ph].
  %%CITATION = ARXIV:1506.03116;%%
  %7 citations counted in INSPIRE as of 11 Aug 2015
 
 %\cite{Abercrombie:2015wmb}
\bibitem{Abercrombie:2015wmb}
  D.~Abercrombie {\it et al.} [ATLAS/CMS DM Forum],
  %``DM Benchmark Models for Early LHC Run-2 Searches: Report of the ATLAS/CMS DM Forum,''
  arXiv:1507.00966 [hep-ex].
  %%CITATION = ARXIV:1507.00966;%%
  %3 citations counted in INSPIRE as of 11 Aug 2015
  
 %\cite{D'Ambrosio:2002ex}
\bibitem{D'Ambrosio:2002ex} 
  G.~D'Ambrosio, G.~F.~Giudice, G.~Isidori and A.~Strumia,
  %``Minimal flavor violation: An Effective field theory approach,''
  Nucl.\ Phys.\ B {\bf 645}, 155 (2002)
  [hep-ph/0207036].
  %%CITATION = HEP-PH/0207036;%%
       
%\cite{Abazov:2003gp}
\bibitem{Abazov:2003gp} 
  V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Search for large extra dimensions in the monojet + missing $E_T$ channel at D\O,''
  Phys.\ Rev.\ Lett.\  {\bf 90}, 251802 (2003)
  [hep-ex/0302014].
  %%CITATION = HEP-EX/0302014;%%
  %78 citations counted in INSPIRE as of 31 Oct 2014    

%\cite{Aaltonen:2012jb}
\bibitem{Aaltonen:2012jb} 
  T.~Aaltonen {\it et al.}  [CDF Collaboration],
  %``A Search for DM in events with one jet and missing transverse energy in $p\bar{p}$ collisions at $\sqrt{s} = 1.96$ TeV,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 211804 (2012)
  [arXiv:1203.0742 [hep-ex]].
  %%CITATION = ARXIV:1203.0742;%%
  %59 citations counted in INSPIRE as of 30 Oct 2014

%\cite{Chatrchyan:2012me} 
\bibitem{Chatrchyan:2012me} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Search for DM and large extra dimensions in monojet events in $pp$ collisions at $\sqrt{s}=7$ TeV,''
  JHEP {\bf 1209}, 094 (2012)
  [arXiv:1206.5663 [hep-ex]].
  %%CITATION = ARXIV:1206.5663;%%
  %173 citations counted in INSPIRE as of 30 Oct 2014
 
  \bibitem{ATLASMONO}
  [ATLAS Collaboration], Conference paper ATLAS-CONF-2012-084.
 
  %\cite{Khachatryan:2014rra}
\bibitem{Khachatryan:2014rra} 
  V.~Khachatryan {\it et al.}  [CMS Collaboration],
  %``Search for DM, extra dimensions, and unparticles in monojet events in proton-proton collisions at $\sqrt{s}$ = 8 TeV,''
  arXiv:1408.3583 [hep-ex].
  %%CITATION = ARXIV:1408.3583;%%
  %14 citations counted in INSPIRE as of 27 Oct 2014

  %\cite{Diehl:2014dda}
\bibitem{Diehl:2014dda} 
  E.~Diehl [ATLAS Collaboration],
  %``The search for DM using monojets and monophotons with the ATLAS detector,''
  AIP Conf.\ Proc.\  {\bf 1604}, 324 (2014).
  %%CITATION = APCPC,1604,324;%%
  %1 citations counted in INSPIRE as of 30 Oct 2014
 
 %\cite{Feng:2005gj}
\bibitem{Feng:2005gj} 
  J.~L.~Feng, S.~Su and F.~Takayama,
  %``Lower limit on DM production at the large hadron collider,''
  Phys.\ Rev.\ Lett.\  {\bf 96}, 151802 (2006)
  [hep-ph/0503117].
  %%CITATION = HEP-PH/0503117;%%
  %60 citations counted in INSPIRE as of 02 Nov 2014

%\cite{Cao:2009uw}
\bibitem{Cao:2009uw} 
  Q.~H.~Cao, C.~R.~Chen, C.~S.~Li and H.~Zhang,
  %``Effective DM Model: Relic density, CDMS II, Fermi LAT and LHC,''
  JHEP {\bf 1108}, 018 (2011)
  [arXiv:0912.4511 [hep-ph]].
  %%CITATION = ARXIV:0912.4511;%%
  %100 citations counted in INSPIRE as of 02 Nov 2014

 %\cite{Beltran:2010ww}
\bibitem{Beltran:2010ww} 
  M.~Beltran, D.~Hooper, E.~W.~Kolb, Z.~A.~C.~Krusberg and T.~M.~P.~Tait,
  %``Maverick DM at colliders,''
  JHEP {\bf 1009}, 037 (2010)
  [arXiv:1002.4137 [hep-ph]].
  %%CITATION = ARXIV:1002.4137;%%
  %153 citations counted in INSPIRE as of 30 Oct 2014

%\cite{Goodman:2010yf}
\bibitem{Goodman:2010yf} 
  J.~Goodman, M.~Ibe, A.~Rajaraman, W.~Shepherd, T.~M.~P.~Tait and H.~B.~Yu,
  %``Constraints on Light Majorana dark Matter from Colliders,''
  Phys.\ Lett.\ B {\bf 695}, 185 (2011)
  [arXiv:1005.1286 [hep-ph]].
  %%CITATION = ARXIV:1005.1286;%%
  %199 citations counted in INSPIRE as of 31 Oct 2014    
    
%\cite{Goodman:2010ku}
\bibitem{Goodman:2010ku} 
  J.~Goodman, M.~Ibe, A.~Rajaraman, W.~Shepherd, T.~M.~P.~Tait and H.~B.~Yu,
  %``Constraints on DM from Colliders,''
  Phys.\ Rev.\ D {\bf 82}, 116010 (2010)
  [arXiv:1008.1783 [hep-ph]].
  %%CITATION = ARXIV:1008.1783;%%
  %265 citations counted in INSPIRE as of 10 Oct 2014

%\cite{Fox:2011pm}
\bibitem{Fox:2011pm}
  P.~J.~Fox, R.~Harnik, J.~Kopp and Y.~Tsai,
 % ``Missing Energy Signatures of DM at the LHC,''
  Phys.\ Rev.\ D {\bf 85} (2012) 056011
  arXiv:1109.4398 [hep-ph].
  %%CITATION = ARXIV:1109.4398;%%
  %202 citations counted in INSPIRE as of 07 Oct 2014
  
  %\cite{Haisch:2012kf}
\bibitem{Haisch:2012kf} 
  U.~Haisch, F.~Kahlhoefer and J.~Unwin,
  %``The impact of heavy-quark loops on LHC DM searches,''
  JHEP {\bf 1307}, 125 (2013)
  [arXiv:1208.4605 [hep-ph]].
  %%CITATION = ARXIV:1208.4605;%%
  %40 citations counted in INSPIRE as of 24 Nov 2014
    
 %\cite{Branco:2011iw}
\bibitem{Branco:2011iw}
  G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
  %``Theory and phenomenology of two-Higgs-doublet models,''
  Phys.\ Rept.\  {\bf 516} (2012) 1
  [arXiv:1106.0034 [hep-ph]].
  %%CITATION = ARXIV:1106.0034;%%
  %433 citations counted in INSPIRE as of 25 mar 2015 
  
  
%\cite{Silveira:1985rk}
\bibitem{Silveira:1985rk}
  V.~Silveira and A.~Zee,
  %``Scalar Phantoms,''
  Phys.\ Lett.\ B {\bf 161} (1985) 136.
  %%CITATION = PHLTA,B161,136;%%
  
%\cite{Schabinger:2005ei}
\bibitem{Schabinger:2005ei}
  R.~Schabinger and J.~D.~Wells,
  %``A Minimal spontaneously broken hidden sector and its impact on Higgs boson physics at the large hadron collider,''
  Phys.\ Rev.\ D {\bf 72} (2005) 093007
  [hep-ph/0509209].
  %%CITATION = HEP-PH/0509209;%%
  
 %\cite{Patt:2006fw}
\bibitem{Patt:2006fw}
  B.~Patt and F.~Wilczek,
  %``Higgs-field portal into hidden sectors,''
  hep-ph/0605188.
  %%CITATION = HEP-PH/0605188;%%

%\cite{Englert:2011yb}
\bibitem{Englert:2011yb} 
  C.~Englert, T.~Plehn, D.~Zerwas and P.~M.~Zerwas,
  %``Exploring the Higgs portal,''
  Phys.\ Lett.\ B {\bf 703}, 298 (2011)
  [arXiv:1106.3097 [hep-ph]].
  %%CITATION = ARXIV:1106.3097;%%
  %77 citations counted in INSPIRE as of 02 Nov 2014

  %\cite{Englert:2013gz}
\bibitem{Englert:2013gz}
  C.~Englert, J.~Jaeckel, V.~V.~Khoze and M.~Spannowsky,
 % ``Emergence of the Electroweak Scale through the Higgs Portal,''
  JHEP {\bf 1304} (2013) 060
  [arXiv:1301.4224 [hep-ph]].
  %%CITATION = ARXIV:1301.4224;%%
  %49 citations counted in INSPIRE as of 09 Oct 2014
  
  %\cite{Hambye:2013dgv}
\bibitem{Hambye:2013dgv}
  T.~Hambye and A.~Strumia,
 % ``Dynamical generation of the weak and DM scale,''
  Phys.\ Rev.\ D {\bf 88} (2013) 055022
  [arXiv:1306.2329 [hep-ph]].
  %%CITATION = ARXIV:1306.2329;%%
  %45 citations counted in INSPIRE as of 09 Oct 2014
  
   %\cite{Carone:2013wla}
\bibitem{Carone:2013wla}
  C.~D.~Carone and R.~Ramos,
  %``Classical scale-invariance, the electroweak scale and vector DM,''
  Phys.\ Rev.\ D {\bf 88} (2013) 055020
  [arXiv:1307.8428 [hep-ph]].
  %%CITATION = ARXIV:1307.8428;%%

%\cite{Khoze:2014xha}
\bibitem{Khoze:2014xha}
  V.~V.~Khoze, C.~McCabe and G.~Ro,
  %``Higgs vacuum stability from the DM portal,''
  JHEP {\bf 1408} (2014) 026
  [arXiv:1403.4953 [hep-ph], arXiv:1403.4953].
  %%CITATION = ARXIV:1403.4953;%%
  %16 citations counted in INSPIRE as of 09 Oct 2014
  
  %\cite{Carena:2004xs}
\bibitem{Carena:2004xs}
  M.~Carena, A.~Daleo, B.~A.~Dobrescu and T.~M.~P.~Tait,
  %``$Z^\prime$ gauge bosons at the Tevatron,''
  Phys.\ Rev.\ D {\bf 70} (2004) 093009
  [hep-ph/0408098].
  %%CITATION = HEP-PH/0408098;%%  

%\cite{Avetisyan:2013onh}
\bibitem{Avetisyan:2013onh} 
  A.~Avetisyan {\it et al.},
  %``Methods and Results for Standard Model Event Generation at $\sqrt{s}$ = 14 TeV, 33 TeV and 100 TeV Proton Colliders (A Snowmass Whitepaper),''
  arXiv:1308.1636 [hep-ex].
  %%CITATION = ARXIV:1308.1636;%%
  %49 citations counted in INSPIRE as of 31 Aug 2015

%\cite{Alwall:2014hca}
\bibitem{Alwall:2014hca}
  J.~Alwall {\it et al.},
  %``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations,''
  JHEP {\bf 1407} (2014) 079
  [arXiv:1405.0301 [hep-ph]].
  %%CITATION = ARXIV:1405.0301;%%

%\cite{Fox:2012ru}
\bibitem{Fox:2012ru} 
  P.~J.~Fox and C.~Williams,
  %``Next-to-Leading Order Predictions for DM Production at Hadron Colliders,''
  Phys.\ Rev.\ D {\bf 87}, no. 5, 054030 (2013)
  [arXiv:1211.6390 [hep-ph]].
  %%CITATION = ARXIV:1211.6390;%%
  
  \bibitem{MCFMweb} 
  J.~M.~Campbell, R.~K.~Ellis and C.~Williams,
MCFM website http://mcfm.fnal.gov

  \bibitem{VBFNLO}
  %\cite{Baglio:2014uba}
%\bibitem{Baglio:2014uba}
  J.~Baglio {\it et al.},
  %``Release Note - VBFNLO 2.7.0,''
  arXiv:1404.3940 [hep-ph];
  %%CITATION = ARXIV:1404.3940;%%
 % 
  %\cite{Arnold:2011wj}
%\bibitem{Arnold:2011wj}
  K.~Arnold {\it et al.},
  %``VBFNLO: A Parton Level Monte Carlo for Processes with Electroweak Bosons -- Manual for Version 2.5.0,''
  arXiv:1107.4038 [hep-ph];
  %%CITATION = ARXIV:1107.4038;%%
  %\cite{Arnold:2008rz}
 %
%\bibitem{Arnold:2008rz}
  K.~Arnold {\it et al.},
  %``VBFNLO: A Parton level Monte Carlo for processes with electroweak bosons,''
  Comput.\ Phys.\ Commun.\  {\bf 180} (2009) 1661
  [arXiv:0811.4559 [hep-ph]].
  %%CITATION = ARXIV:0811.4559;%%
  
  %\cite{Sjostrand:2007gs}
\bibitem{Sjostrand:2007gs} 
  T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
  %``A Brief Introduction to PYTHIA 8.1,''
  Comput.\ Phys.\ Commun.\  {\bf 178}, 852 (2008)
  [arXiv:0710.3820 [hep-ph]].
  %%CITATION = ARXIV:0710.3820;%%

\bibitem{Ball:2014uwa}
  R.~D.~Ball {\it et al.} [NNPDF Collaboration],
  %``Parton distributions for the LHC Run II,''
  JHEP {\bf 1504} (2015) 040
  [arXiv:1410.8849 [hep-ph]].
  %%CITATION = ARXIV:1410.8849;%%
  %65 citations counted in INSPIRE as of 31 Aug 2015  

 %\cite{Backovic:2015soa}
\bibitem{Backovic:2015soa} 
  M.~Backovic, M.~Krämer, F.~Maltoni, A.~Martini, K.~Mawatari and M.~Pellen,
  %``Higher-order QCD predictions for DM production at the LHC in simplified models with s-channel mediators,''
  arXiv:1508.05327 [hep-ph].
  %%CITATION = ARXIV:1508.05327;%%
  
  %\cite{Mattelaer:2015haa}
\bibitem{Mattelaer:2015haa} 
  O.~Mattelaer and E.~Vryonidou,
  %``Dark matter production through loop-induced processes at the LHC: the s-channel mediator case,''
  Eur.\ Phys.\ J.\ C {\bf 75}, no. 9, 436 (2015)
  [arXiv:1508.00564 [hep-ph]].
  %%CITATION = ARXIV:1508.00564;%%
  %2 citations counted in INSPIRE as of 23 Oct 2015
  
  \bibitem{Butler:2020886}
  Butler, J and Contardo, D and Klute, M and Mans, J and Silvestris, L,
  CERN-LHCC-2015-010. LHCC-P-008.

\bibitem{ATLAS:1502664}
  ATLAS,  Collaboration,
  CERN-LHCC-2012-022. LHCC-I-023.

  
 %\cite{Khachatryan:2014gga}
\bibitem{Khachatryan:2014gga}
  V.~Khachatryan {\it et al.} [CMS Collaboration],
  %``Performance of the CMS missing transverse momentum reconstruction in pp data at $\sqrt{s}$ = 8 TeV,''
  JINST {\bf 10} (2015) 02,  P02006 
  [arXiv:1411.0511 [physics.ins-det]].
  %%CITATION = ARXIV:1411.0511;%%
  %12 citations counted in INSPIRE as of 28 Aug 2015     
  
  \bibitem{CMSJet}
  V.~Khachatryan {\it et al.} [CMS Collaboration], 
  JINST {\bf 6} (2011), 11002 
  [ arXiv:1107.4277v1 [physics.ins-det]].
  
 %\cite{CMS:2015jha}
\bibitem{CMS:2015jha}
  CMS Collaboration [CMS Collaboration],
  %``Search for New Physics in the V-jet + MET final state,''
  CMS-PAS-EXO-12-055.
  %%CITATION = CMS-PAS-EXO-12-055;%%
 
%\cite{CMS:2015fla}
\bibitem{CMS:2015fla}
  CMS Collaboration [CMS Collaboration],
  %``Search for DM direct production using razor
  variables in events with two or more jets in pp collisions at 8
  TeV,''
  CMS-PAS-EXO-14-004.
  %%CITATION = CMS-PAS-EXO-14-004;%%
  %4 citations counted in INSPIRE as of 28 Aug 2015

%\cite{CMS:2012ova}
\bibitem{CMS:2012ova}
  CMS Collaboration [CMS Collaboration],
  %``Search for Supersymmetry in hadronic final states using MT2 with the CMS detector at 7 TeV,''
  CMS-PAS-SUS-12-002.
  %%CITATION = CMS-PAS-SUS-12-002;%%
  %22 citations counted in INSPIRE as of 28 Aug 2015
  
%\cite{Read:2002hq}
\bibitem{Read:2002hq} 
  A.~L.~Read,
  %``Presentation of search results: The CL(s) technique,''
  J.\ Phys.\ G {\bf 28}, 2693 (2002).
  %%CITATION = JPAGA,G28,2693;%%
  %1173 citations counted in INSPIRE as of 19 août 2015    

\bibitem{Cowan:2010js} 
  G.~Cowan, K.~Cranmer, E.~Gross and O.~Vitells,
  %``Asymptotic formulae for likelihood-based tests of new physics,''
  Eur.\ Phys.\ J.\ C {\bf 71}, 1554 (2011)
  [Eur.\ Phys.\ J.\ C {\bf 73}, 2501 (2013)]
  [arXiv:1007.1727 [physics.data-an]].
  %%CITATION = ARXIV:1007.1727;%%
  %764 citations counted in INSPIRE as of 19 Aug 2015    

  %\cite{Cheng:2012qr}
\bibitem{Cheng:2012qr} 
  H.~Y.~Cheng and C.~W.~Chiang,
  %``Revisiting Scalar and Pseudoscalar Couplings with Nucleons,''
  JHEP {\bf 1207}, 009 (2012)
  [arXiv:1202.1292 [hep-ph]].
  %%CITATION = ARXIV:1202.1292;%%
  %21 citations counted in INSPIRE as of 24 Oct 2014


%\cite{Buchmueller:2013dya}
\bibitem{Buchmueller:2013dya}
  O.~Buchmueller, M.~J.~Dolan and C.~McCabe,
  %``Beyond Effective Field Theory for DM Searches at the LHC,''
  JHEP {\bf 1401} (2014) 025
  [arXiv:1308.6799 [hep-ph]].
  %%CITATION = ARXIV:1308.6799;%%
  
\bibitem{Kurylov:2003ra} 
  A.~Kurylov and M.~Kamionkowski,
  %``Generalized analysis of weakly interacting massive particle searches,''
  Phys.\ Rev.\ D {\bf 69}, 063503 (2004)
  [hep-ph/0307185].
  %%CITATION = HEP-PH/0307185;%%

%\cite{Hisano:2010ct}
\bibitem{Hisano:2010ct} 
  J.~Hisano, K.~Ishiwata and N.~Nagata,
  %``Gluon contribution to the DM direct detection,''
  Phys.\ Rev.\ D {\bf 82}, 115007 (2010)
  [arXiv:1007.2601 [hep-ph]].
  %%CITATION = ARXIV:1007.2601;%%
  
%\cite{Cheung:2013pfa}
\bibitem{Cheung:2013pfa} 
  K.~Cheung, C.~T.~Lu, P.~Y.~Tseng and T.~C.~Yuan,
  %``Collider Constraints on the DM Interpretation of the CDMS II Results,''
  arXiv:1308.0067 [hep-ph].
  %%CITATION = ARXIV:1308.0067;%%

  %\cite{Crivellin:2013ipa}
\bibitem{Crivellin:2013ipa}
  A.~Crivellin, M.~Hoferichter and M.~Procura,
  %``Accurate evaluation of hadronic uncertainties in spin-independent WIMP-nucleon scattering: Disentangling two- and three-flavor effects,''
  Phys.\ Rev.\ D {\bf 89} (2014) 054021
  [arXiv:1312.4951 [hep-ph]].
  %%CITATION = ARXIV:1312.4951;%%

\bibitem{Hoferichter:2015dsa}
  M.~Hoferichter, J.~Ruiz de Elvira, B.~Kubis and U.~G.~Meißner,
  %``High-precision determination of the pion-nucleon $\sigma$-term from Roy-Steiner equations,''
  Phys.\ Rev.\ Lett.\  {\bf 115} (2015) 092301
  [arXiv:1506.04142 [hep-ph]].
  %%CITATION = ARXIV:1506.04142;%%
  %5 citations counted in INSPIRE as of 31 Aug 2015
  
  %\cite{Cushman:2013zza}
\bibitem{Cushman:2013zza}
  P.~Cushman {\it et al.},
  %``Working Group Report: WIMP DM Direct Detection,''
  arXiv:1310.8327 [hep-ex].
  %%CITATION = ARXIV:1310.8327;%%
  %107 citations counted in INSPIRE as of 31 Aug 2015
  
  %\cite{Ackermann:2011wa}
\bibitem{Ackermann:2011wa} 
  M.~Ackermann {\it et al.}  [Fermi-LAT Collaboration],
  %``Constraining DM Models from a Combined Analysis of Milky Way Satellites with the Fermi Large Area Telescope,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 241302 (2011)
  [arXiv:1108.3546 [astro-ph.HE]].
  %%CITATION = ARXIV:1108.3546;%%
  %362 citations counted in INSPIRE as of 27 Oct 2014

%\cite{Abdo:2010ex}
\bibitem{Abdo:2010ex} 
  A.~A.~Abdo {\it et al.}  [Fermi-LAT Collaboration],
  %``Observations of Milky Way Dwarf Spheroidal galaxies with the Fermi-LAT detector and constraints on DM models,''
  Astrophys.\ J.\  {\bf 712}, 147 (2010)
  [arXiv:1001.4531 [astro-ph.CO]].
  %%CITATION = ARXIV:1001.4531;%%
  %199 citations counted in INSPIRE as of 31 Oct 2014

%\cite{Zheng:2010js}
\bibitem{Zheng:2010js} 
  J.~M.~Zheng, Z.~H.~Yu, J.~W.~Shao, X.~J.~Bi, Z.~Li and H.~H.~Zhang,
  %``Constraining the interaction strength between DM and visible matter: I. fermionic DM,''
  Nucl.\ Phys.\ B {\bf 854}, 350 (2012)
  [arXiv:1012.2022 [hep-ph]].
  %%CITATION = ARXIV:1012.2022;%%
  %37 citations counted in INSPIRE as of 27 Oct 2014

%\cite{Boehm:2014hva}
\bibitem{Boehm:2014hva} 
  C.~Boehm, M.~J.~Dolan, C.~McCabe, M.~Spannowsky and C.~J.~Wallace,
  %``Extended gamma-ray emission from Coy DM,''
  JCAP {\bf 1405}, 009 (2014)
  [arXiv:1401.6458 [hep-ph]].
  %%CITATION = ARXIV:1401.6458;%%
 

\end{thebibliography}


==> 02-DM/DM_SM_portal_4/declare.tex <==

\def\contentsname{{\normalsize Content}}
\def\tablename{Table}
\def\figurename{Figure}

\def\pveto{P_\text{veto}}
\def\nj{n_\text{jets}}
\def\meff{m_\text{eff}}
\def\ptmin{p_T^\text{min}}
\def\gtot{\Gamma_\text{tot}}
\def\as{\alpha_s}
\def\az{\alpha_0}
\def\gz{g_0}
\def\w{\vec{w}}
\def\sdag{\Sigma^{\dag}}
\def\s{\Sigma}
\newcommand{\tr}{\text{track}}
\newcommand{\lsp}{{\tilde \chi}}
\newcommand{\mlsp}{m_{\tilde \chi}}
\newcommand{\psib}{\overline{\psi}}
\newcommand{\Psib}{\overline{\Psi}}
%\newcommand{\dslash}{\not{\hbox{\kern-3pt $\partial$}}}
%\newcommand{\Dslash}{\not{\hbox{\kern-3pt $D$}}}
%\def\one{\leavevmode\hbox{\small1\kern-7.3pt\normalsize1}}
%%\def\one{I}
\newcommand\one{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
\newcommand{\Mpl}{M_\text{Pl}}
%\def\dslash{\not{\hbox{\kern-4pt $\partial$}}}
%\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\newcommand{\p}{\partial}
\newcommand{\mat}{\mathcal{M}}
\newcommand{\lag}{\mathcal{L}}
\newcommand{\ord}{\mathcal{O}}
\newcommand{\ope}{\mathcal{O}}
\newcommand{\qqquad}{\qquad \qquad}
\newcommand{\qqqquad}{\qquad \qquad \qquad}
 
\newcommand{\ds}{\displaystyle}
\newcommand{\qb}{\bar{q}}
\newcommand{\matx}{|\mathcal{M}|^2}
%\newcommand{\mat}{\mathcal{M}}
%\newcommand{\slashed}[1]{\ensuremath{{#1}{\!}{\!}{\!}{\!}{\:}/}}
\newcommand{\really}{\stackrel{!}{=}}
\newcommand{\msbar}{\overline{\text{MS}}}
\newcommand{\qns}{f_q^\text{NS}}
\newcommand{\lqcd}{\Lambda_\text{QCD}}
\newcommand{\met}{\slashchar{p}_T}
\newcommand{\pmiss}{\slashchar{\vec{p}}_T}

\newcommand{\sq}{\tilde{q}}
\newcommand{\go}{\tilde{g}}
\newcommand{\st}[1]{\tilde{t}_{#1}}
\newcommand{\stb}[1]{\tilde{t}_{#1}^*}
\newcommand{\nz}[1]{\tilde{\chi}_{#1}^0}
\newcommand{\cp}[1]{\tilde{\chi}_{#1}^+}
\newcommand{\cm}[1]{\tilde{\chi}_{#1}^-}
\newcommand{\CP}{CP}

% all the masses 
\providecommand{\mg}{m_{\tilde{g}}}
\providecommand{\mst}[1]{m_{\tilde{t}_{#1}}}
\newcommand{\msn}[1]{m_{\tilde{\nu}_{#1}}}
\newcommand{\mch}[1]{m_{\tilde{\chi}^+_{#1}}}
\newcommand{\mne}[1]{m_{\tilde{\chi}^0_{#1}}}
\newcommand{\msb}[1]{m_{\tilde{b}_{#1}}}
\newcommand{\vsm}{\ensuremath{v_\text{SM}}}

% units of measure
\newcommand{\toolfont}[1]{\texttt{#1}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ab}{\text{ab}}
\newcommand{\pb}{\text{pb}}
\newcommand{\br}{\text{BR}}
\newcommand{\sign}{\text{sign}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\ipb}{\text{pb}^{-1}}

% really great macro by Chris Lester
\def\slashchar#1{\setbox0=\hbox{$#1$}           % set a box for #1
   \dimen0=\wd0                                 % and get its size
   \setbox1=\hbox{/} \dimen1=\wd1               % get size of /
   \ifdim\dimen0>\dimen1                        % #1 is bigger
      \rlap{\hbox to \dimen0{\hfil/\hfil}}      % so center / in box
      #1                                        % and print #1
   \else                                        % / is bigger
      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}   % so center #1
      /                                         % and print /
   \fi}
\newcommand{\dslash}{\slashchar{\partial}}
\newcommand{\Dslash}{\slashchar{D}}

\newcommand{\eg}{\textsl{e.g.}\;}
\newcommand{\ie}{\textsl{i.e.}\;}
\newcommand{\etal}{\textsl{et al}\;}
%\DeclareMathOperator{\tr}{Tr}

% maximal number of floating environments on each page 
\setlength{\floatsep}{0pt}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{1}
\setcounter{totalnumber}{1}
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.0}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\rig}{\rightarrow}
\newcommand{\lrig}{\longrightarrow}
\renewcommand{\d}{{\text{d}}}
\newcommand{\gl}[1]{(\ref{#1})}
\newcommand{\ta}[2]{ \frac{ {\text{d}} #1 } {{\text{d}} #2}}
\newcommand{\mc}{\mathcal}
\newcommand{\mr}{\mathrm}
\newcommand{\ep}{\varepsilon}
\newcommand{\eps}{\varepsilon}
%\renewcommand{\vec}{\bf}
\newcommand{\emt}{$\times 10^{-3}$}
\newcommand{\emfo}{$\times 10^{-4}$}
\newcommand{\emfi}{$\times 10^{-5}$}

\newcommand{\revision}[1]{{\bf{}#1}}

\newcommand{\sw}{\ensuremath{s_w}}
\newcommand{\cw}{\ensuremath{c_w}}
\newcommand{\swd}{\ensuremath{s^2_w}}
\newcommand{\cwd}{\ensuremath{c^2_w}}


